EMR-AGENT: Automating Cohort and Feature Extraction from EMR Databases

Machine learning models for clinical prediction rely on structured data extracted from Electronic Medical Records (EMRs), yet this process remains dominated by hardcoded, database-specific pipelines for cohort definition, feature selection, and code mapping. These manual efforts limit scalability, reproducibility, and cross-institutional generalization. To address this, we introduce EMR-AGENT (Automated Generalized Extraction and Navigation Tool), an agent-based framework that replaces manual rule writing with dynamic, language model-driven interaction to extract and standardize structured clinical data. Our framework automates cohort selection, feature extraction, and code mapping through interactive querying of databases. Our modular agents iteratively observe query results and reason over schema and documentation, using SQL not just for data retrieval but also as a tool for database observation and decision making. This eliminates the need for hand-crafted, schema-specific logic. To enable rigorous evaluation, we develop a benchmarking codebase for three EMR databases (MIMIC-III, eICU, SICdb), including both seen and unseen schema settings. Our results demonstrate strong performance and generalization across these databases, highlighting the feasibility of automating a process previously thought to require expert-driven design. The code will be released publicly at https://github.com/AITRICS/EMR-AGENT/tree/main. For a demonstration, please visit our anonymous demo page: https://anonymoususer-max600.github.io/EMR_AGENT/

==> Sections/table_datasets.tex <==
\begin{table}[!h]
   \centering
   \caption{Types and purposes of datasets used in study.}
   \label{tab_datasets}
   \begin{tabular}{ccccc}
   \toprule
    \textbf{Dataset} & \textbf{Version} & \textbf{Published} & \textbf{Use} & \textbf{Purpose} \\ \hline
       MIMIC-III \cite{johnson2016mimic} & 1.4 & May, 2016 & $\checkmark$ & EMR database environment \\
       eICU \cite{pollard2019eicu} & 2.0 & Apr, 2019 & $\checkmark$ & EMR database environment \\
       SICdb \cite{rodemund2023salzburg} & 1.0.8 & Sep, 2024 & $\checkmark$ & EMR database environment \\
       HiRID\cite{faltys2021hirid} & 1.1.1 & Feb, 2021 & $\triangle$ & Reference for the feature list \\
   \bottomrule
   \end{tabular}
\end{table}


